DragD3D: Realistic Mesh Editing with Rigidity Control Driven by 2D Diffusion Priors

Direct mesh editing and deformation are key components in the geometric modeling and animation pipeline. Mesh editing methods are typically framed as optimization problems combining user-specified vertex constraints with a regularizer that determines the position of the rest of the vertices. The choice of the regularizer is key to the realism and authenticity of the final result. Physics and geometry-based regularizers are not aware of the global context and semantics of the object, and the more recent deep learning priors are limited to a specific class of 3D object deformations. Our main contribution is a vertex-based mesh editing method called DragD3D based on (1) a novel optimization formulation that decouples the rotation and stretch components of the deformation and combines a 3D geometric regularizer with (2) the recently introduced DDS loss which scores the faithfulness of the rendered 2D image to one from a diffusion model. Thus, our deformation method achieves globally realistic shape deformation which is not restricted to any class of objects. Our new formulation optimizes directly the transformation of the neural Jacobian field explicitly separating the rotational and stretching components. The objective function of the optimization combines the approximate gradients of DDS and the gradients from the geometric loss to satisfy the vertex constraints. Additional user control over desired global shape deformation is made possible by allowing explicit per-triangle deformation control as well as explicit separation of rotational and stretching components of the deformation. We show that our deformations can be controlled to yield realistic shape deformations that are aware of the global context of the objects, and provide better results than just using geometric regularizers.

==> TODO.tex <==


4) Ablation --> 

A result with only T

1) Re organize the paper so that we can fit: put the dragon with the animals and bring the castle and chair up
This way we can fit also teh ablation figure at teh bottom of teh  gallery of results 2

2) Do we want to compare with ARAP as a direcrt reguralizer since we do with T?

3) What are the new meshes without texture

4) Do we have the correct template, there are som issues on some pages

5) I would remove the second cat, it does not add anything and thwe results I noticed now it is not as good from a symmetry point of view


6) Need letters for all rows in the figures



Questions/todo

1) Reviewer continuity? - NO - DONE
2) In the intro the 1,2,3 strategoes shoudl have end of lines after? - KEEP
3) Emphasize that the rigidity map is optional and it is very easy to specify - TODO
4) Castle: stretching plus mask at the same time - TODO



7) Review the keywords in the submission - DONE

8) Review the video - a few issues to be discussed w Tianhao - DONE


10) Limitations: even finer control of the weights instead of binary mask - NO, DONE


11) Video options to make it smaller - DONE



-----

PRIORITYL

14) Conclusions section Need to reqeuite the first paragraph of conclusion to reflect the rigidity mask - DONE 

 12) - Car is 2000 iterations - DONE

15) comparison stuff

Global: symmetry (car, cat ears)
      postures --> dragon and elephant


      Local: cat face, back of the chair, car window, lantern, (rigidity masks objects)



      5) Check figure captions - TODO

      6) sections 4.3, 4.4, 5

     

13) - Emphasize the multiple views stuff


Check w Tiqahao:
1) VIDEO
2) Arrows in the figures - DONE


Latest Agenda


15) Work the nice rebuttal phrasing in the intro and conclusion - OK

14) Did the elep[hant raise its head? very difficult to see - rephrase it a bit
Do we mention the bag? not our best result? - remove from TEXT


16) Captions? - DONE

17) Review Eugene's comments - OK
